Social Interactions or Business Transactions? What customer reviews disclose about Airbnb marketplace

Airbnb is one of the most successful examples of sharing economy marketplaces. With rapid and global market penetration, understanding its attractiveness and evolving growth opportunities is key to plan business decision making. There is an ongoing debate, for example, about whether Airbnb is a hospitality service that fosters social exchanges between hosts and guests, as the sharing economy manifesto originally stated, or whether it is (or is evolving into being) a purely business transaction platform, the way hotels have traditionally operated. To answer these questions, we propose a novel market analysis approach that exploits customers' reviews. Key to the approach is a method that combines thematic analysis and machine learning to inductively develop a custom dictionary for guests' reviews. Based on this dictionary, we then use quantitative linguistic analysis on a corpus of 3.2 million reviews collected in 6 different cities, and illustrate how to answer a variety of market research questions, at fine levels of temporal, thematic, user and spatial granularity, such as (i) how the business vs social dichotomy is evolving over the years, (ii) what exact words within such top-level categories are evolving, (iii) whether such trends vary across different user segments and (iv) in different neighbourhoods.

==> sec_preliminary.tex <==
\section{Preliminary investigation}

\begin{itemize}
\item To have a preliminary view on the topics discussed on the Airbnb reviews and how these topics are evolving over time, we bin reviews by a time span of 3 years: reviews released in early years (years between 2010--2012) vs. reviews released in late years (years between 2017--2019). For each word (1-gram) $w$ and each temporal bin of 3 years, $t_{2010\_12}$ vs. $t_{2017\_19}$, we compute the corresponding logarithmically scaled term frequencies $tf_{2010\_12}(w)$ and $tf_{2017\_19}(w)$. Finally, for each word $w$, we compute the term frequency gain as:
	\begin{equation}
	tf_{gain}(w) = \frac{tf_{2017\_19}(w)}{tf_{2010\_12}(w)} 
	\label{eq:tf_gain}
	\end{equation}
which is the ratio between the two term frequencies. Since each term frequency is normalised in [0,1], this metric is able to detect which words have been over-used in the late years compared to the early ones ($tf_{gain}>1$), and vice versa ($tf_{gain}<1$). 

\item Table~\ref{tab:TFgain} shows the top-10 words having, in average across all cities, the highest and the lowest term frequency gain. To avoid displaying very rare words, we filtered out from our visualisation all words having a global term frequency, across all years, lower than $10^{-5}$. 

\item Insight from Table~\ref{tab:TFgain}: new terms are used in late years (e.g., lyft, uber). This is not surprising since these services barely existed in the early years. Beside this, more terms -- which are intuitively more business -- have been used in the late years (e.g., sparkling, reactive, responses) compare the terms used in the early years -- which are more social (e.g., friend, spent, pleasure, meet, charming, him). 

\begin{table}[!ht]
   \centering
   \mytablesize 
   \begin{tabular}{lr | lr}
   \em Top terms & $tf_{gain}(t)$ & \em Bottom terms & $tf_{gain}(t)$ \\
   \hline \hline
   lyft      & 127.5  & friend      & 0.42 \\
   uber      & 16.9   & spent       & 0.43 \\
   airbnbs   & 13.9   & pleasure    & 0.46 \\
   skybus    & 13.3   & week        & 0.48 \\
   superhost & 13.1   & information & 0.51 \\
   sparkling & 11.2   & meet        & 0.51 \\
   lockbox   & 9.2    & charming    & 0.52 \\
   coles     & 8.8    & first       & 0.54 \\
   reactive  & 6.7    & him         & 0.55 \\
   responses & 6.4    & hope        & 0.56 \\
   \hline \hline
   \end{tabular}
   \caption{Words having the top/bottom 10 term frequency gain}
   \label{tab:TFgain}
\end{table}

\item This preliminary analysis shows that there is evidence that social interactions are rapidly decreasing on Airbnb. 
%There is also some early evidence that the shift is global. That is why we set out to analyse Airbnb data over time on different cities located in 3 different countries/continents to test those preliminary evidences for the first time.
\end{itemize}


